Elementary exposition of realizing phase space structures relevant to chemical reaction dynamics

In this article, we review the analytical and numerical approaches for computing the phase space structures in two degrees-of-freedom Hamiltonian systems that arise in chemical reactions. In particular, these phase space structures are the unstable periodic orbit associated with an index-1 saddle, the periodic orbit dividing surface, and the stable and unstable invariant manifolds of the unstable periodic orbit. We review the approaches in the context of a two degrees-of-freedom Hamiltonian with a quartic potential coupled with a quadratic potential. We derive the analytical form of the phase space structures for the integrable case and visualize their geometry on the three dimensional energy surface. We then investigate the bifurcation of the dividing surface due to the changes in the parameters of the potential energy. We also review the numerical method of \emph{turning point} and present its new modification called the \emph{turning point based on configuration difference} for computing the unstable periodic orbit in two degrees-of-freedom systems. These methods are implemented in the open-source python package, UPOsHam~\cite{Lyu2020}.

==> scrapyard.tex <==
\begin{abstract}
A two Degree-of-Freedom(DoF) uncoupled Hamiltonian system is considered where bifurcation of dividing surface(DS) can occur for certain value of parameters. Visualisation of the geometrical structures of the Hamiltonian system, trajectories on the manifold and bifurcation analysis are presented. In this system, analytical form of the phase space structures can be obtained including a Normally Hyperbolic Invariant Manifold(NHIM). A method called turning point used to compute the NHIM is also discussed.
\end{abstract}
In this case, there are special points that the system is in equilibrium called equilibrium points
In the neighbourhood of the equilibrium points, trajectories are usually surrounded, or go towards these points. Saddle point is one type of equilibrium points and its generalisation to higher dimensions is called a Normally Hyperbolic Invariant Manifold (NHIM)~\cite{Wiggins1990,Wiggins1994}. Saddle point is one type of equilibrium points and its generalisation to higher dimensions is called a Normally Hyperbolic Invariant Manifold (NHIM)

In order to understand a complex system with many DoF, we need to understand the system well when the dimension of the phase space is low, such as 2. 

and the time evolution of coordinates is represented by trajectories

We say that each pair $(q_i,p_i)$ has its own Degree-of-Freedom (DoF) to move within the system and the whole dynamics happen in the place, called phase space. 

In chemistry, a molecule is a set of atoms that is bounded by some chemical bonds and a reaction occurs when the bonds between atoms break. Mathematically we can describe the bond length of atoms as reaction coordinates $q_1,...,q_n$ and set $q_i$ to $\infty$ to represent a particular bond is breaking. 


given a particular $q_i$, 


so it turns out that using Hamiltonian mechanics is the most appropriate. 


In chemical reaction dynamics~\cite{NHIMinchem}, the NHIM plays a fundamental role that it's used to construct a special surface, call the Dividing surface(DS). The DS separates the energy surface into reactants component and products component. 



Other phase space structures associated to the NHIM, such as its stable and the unstable manifolds act as barriers between different types of trajectories in phase space. For complicated systems, we do not have an analytical form for the stable and unstable manifolds, location of the NHIM is a basis for computing the stable and unstable manifolds numerically. The NHIM is also used in an action integral to compute the directional flux through the DS~~\cite{waalkens2004direct,Waalkens2005} which is used to compute the reaction rate~\cite{Ezra2009}.


allowed in $ q_1-p_1$ (or $ x-p_x$) plane

more complicated example 

an example in this article

example is interesting

because it allows for 

We will show that the NHIM has an analytical form which is a one-dimensional unstable periodic orbit(UPO) and it is easy to visualise it in the phase space. However, in more complicated situation, we can not obtain an analytical form for the NHIM and numerical methods need to be applied. 


There are existing methods for numerical computing UPOs,


Turning point method~\cite{Pollak1980} is a simple method that is based on the geometry of the UPO. It assumes that there are two trajectories starting on the equipotential line in the configuration space with some given energy. It also assumes that the two initial conditions are close to the NHIM. As the trajectories evolve in time, they will reach some turning points and change their directions before they get to the different side of the equipotential line. If the trajectories turn in different directions, the NHIM must exist between the two trajectories. Different conditions can be used to check whether the trajectories turn in opposite directions or not. Turning point method uses a dot product condition and turning point based on configuration difference method uses the configuration difference between the turning points and the starting points. 


case by case 


results in having 2 NHIMs and 2 DSs associated to each NHIM

The DSs are viewed as the boundary between reactants, products and another region where we call it 'intermediate' region.


Unfortunately, the structure of the NHIM and the stable and unstable manifolds associated to the NHIM in the coupled system does not have an analytical form and we can only use numerical methods to find it. However, the method of turning point and turning point based on the configuration difference can still be used to find the position of the NHIM. Details can be found at ~\cite{Lyu2020}.

